Open Intent Discovery through Unsupervised Semantic Clustering and Dependency Parsing

Intent understanding plays an important role in dialog systems, and is typically formulated as a supervised learning problem. However, it is challenging and time-consuming to design the intents for a new domain from scratch, which usually requires a lot of manual effort of domain experts. This paper presents an unsupervised two-stage approach to discover intents and generate meaningful intent labels automatically from a collection of unlabeled utterances in a domain. In the first stage, we aim to generate a set of semantically coherent clusters where the utterances within each cluster convey the same intent. We obtain the utterance representation from various pre-trained sentence embeddings and present a metric of balanced score to determine the optimal number of clusters in K-means clustering for balanced datasets. In the second stage, the objective is to generate an intent label automatically for each cluster. We extract the ACTION-OBJECT pair from each utterance using a dependency parser and take the most frequent pair within each cluster, e.g., book-restaurant, as the generated intent label. We empirically show that the proposed unsupervised approach can generate meaningful intent labels automatically and achieve high precision and recall in utterance clustering and intent discovery.

==> intent-discovery-archive/approach.tex <==
%%%%%%%%%%%%%%%%%%
\section{Approach}
We propose a two-stage approach for \textit{open intent discovery}: (1) semantic-based unsupervised clustering and (2) parsing-based label generation, as shown in Figure~\ref{fig:architecture}. The first stage consists of deriving semantic representations and performing unsupervised clustering, while the second stage adopts a dependency parser to extract ACTION-OBJECT pairs and generate intent labels in an automatic manner.
\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/architecture.pdf}
    \vspace{-1em}
    \caption{The two-stage approach for open intent discovery.}
    \label{fig:architecture}
\end{figure}

\vspace{-1.5em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Semantic Representation}
Pre-trained language models such as BERT have been successfully adopted in various downstream NLP tasks.
Reimers and Gurevych \cite{reimers2019sentencebert} presents the Sentence-BERT (SBERT), which uses a Siamese network structure to derive sentence embeddings that are particularly suited for efficient semantic similarity search and clustering.
We represent each utterance with its semantic vector using the SBERT model pre-trained from different tasks and datasets, such as paraphrase generation, natural language inference, semantic textual similarity, etc.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Unsupervised Clustering}
We use the $K$-means algorithm to learn $K$ clusters automatically. For a given utterance represented as a semantic vector $\mathbf {x}$, the objective of $K$-means is to find a set of clusters $C={C_1, C_2, \ldots, C_K}$ which minimizes the within-cluster sum of square errors, as defined in Equation~(\ref{eq:k-means}), where $\boldsymbol{\mu}_i$ is the mean of the examples in the cluster of $C_i$. Note that the $K$-means algorithm tends to generate clusters of similar sizes.
\vspace{-0.5em}
\begin{align} \label{eq:k-means}
    \underset {\mathbf {C} }{\operatorname {arg\,min} }\sum _{i=1}^{K}\sum _{\mathbf {x} \in C_{i}}\left\|\mathbf {x} -{\boldsymbol {\mu }}_{i}\right\|^{2}
\end{align}
However, there is a challenge in choosing an optimal $K$.
We introduce a metric named \textit{balanced score} to choose the optimal number of clusters. It extends the Silhouette score \cite{rousseeuw1987silhouettes} by a penalty term to encourage a set of clusters with the similar number of examples, defined as follows:
% The following equations define the balanced score $b(i)$. 
Let $C_i$ denote the assigned cluster of the data point $i$ (i.e., $i \in C_i$), then $a(i)$ measures the mean distance between $i$ and all other data points in the same cluster $C_i$, while $b(i)$ is the smallest mean distance of $i$ to all points in any other cluster. $s(i)$ is defined as the conventional Silhouette score, whereas $l(i)$ extends $s(i)$ by a penalty term to encourage clusters of similar sizes. As defined in Equation~(\ref{eq:penalty}), $\sum_{k=1}^K \left |\frac{|C_k|}{N} - \frac{1}{K} \right|$ becomes 0 if all the clusters have the same number of examples, and becomes larger otherwise, and the ratio of $\frac{\sigma}{\mu}$ is defined as the \textit{coefficient of variation} (cv) \cite{everitt2002cambridge} to measure the dispersion of the cluster sizes having the the standard deviation $\sigma$ and the mean $\mu$. We also use the coefficient $\lambda$, ranging from 0 to 1, to scale the penalty term.  We will empirically show that the penalty term works well with the $K$-means algorithm on a balanced dataset, since both of them prefer the clusters of similar sizes. 

\vspace{-1.3em}
\begin{align}
a(i) &= \frac{1}{|C_i|-1} \sum_{j\in C_i, i\neq j} d(i, j) \\
b(i) &= \min_{k\neq i} \frac{1}{|C_k|} \sum_{j\in C_k} d(i, j) \\
s(i) &= \frac{b(i)-a(i)}{\max\{a(i), b(i)\}} \\
% b(i) &= \frac{b(i)-a(i)}{max\{a(i), b(i)\}} - \lambda \sum_{i=1} ^K |\frac{C_i}{N} - \frac{1}{K}|
% b(i) &= s(i) - \frac{1}{\sqrt{K}} \sum_{i=1} ^K \left |\frac{|C_i|}{N} - \frac{1}{K} \right|
% b(i) &= s(i) - \lambda\sum_{i=1} ^K \left |\frac{|C_i|}{N} - \frac{1}{K} \right| \label{eq:penalty}
l(i) &= s(i) - \lambda \frac{\sigma}{\mu} \sum_{k=1} ^K \left |\frac{|C_k|}{N} - \frac{1}{K} \right| \label{eq:penalty}
\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Label Generation}
Given the $K$ clusters obtained in the previous clustering stage, the most frequent ACTION-OBJECT pair within each cluster is taken as the cluster label, e.g., \texttt{play-music}, \texttt{book-restaurant}.
For each utterance in a cluster, we extract an ACTION-OBJECT pair using the \texttt{dobj} rule parsed from the spaCy dependency parser\cite{honnibal2015improved}, where the ACTION word is a verb and the OBJECT word is a noun or a noun phrase. If there is no such pair in an incomplete or overly short utterance, either ACTION or OBJECT is denoted as NONE. Since we generate the cluster label using the most frequent ACTION-OBJECT pair, the final label for a cluster will not be affected by these incomplete pairs. 
% Besides, we filter out the OBJECT words which are numbers or the ACTION words of be (am, is are), to extract the words with clear semantics.
Besides, we filter out the OBJECT words which are numbers to extract the words with clear semantics.
In the ideal cases, the most frequent ACTION-OBJECT pair within each cluster serves as a good label for the cluster, e.g., \texttt{book-restaurant}. In extreme cases, if there is not even a single ACTION-OBJECT pair available, we take the most frequent ACTION word and the most frequent OBJECT word and concatenate them as the cluster label.


==> intent-discovery-archive/conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}

The paper presents an unsupervised data-driven framework which simultaneously solves two tasks in the problem of open intent discovery: (1) discovering all intents from an unlabeled goal-oriented dialog corpus and (2) recognizing the corresponding intent for each utterance from the corpus. To estimate the number of intents, we introduce the balanced score which extends the Silhouette score by adding a penalty term to encourage balance among the intent clusters. We design a rule-based method to generate interpretable labels in the form of ACTION-OBJECT for the discovered intents based on the results of dependency parsing. This can greatly save the costs of manual labeling for developing the intent understanding module in a dialog system. We evaluated the proposed framework with the SNIPS dataset and found that the discovered intents match exactly with the manually labeled intents. Also, the intents of the utterances are recognized in high precision and recall, showing that the proposed framework is effective in intent discovery.

==> intent-discovery-archive/experiments.tex <==
\section{Experiments}

\subsection{Experimental Setup}
To evaluate the proposed framework, we use the publicly available SNIPS\cite{coucke2018snips} dataset which has 13,784 sentences and 7 ground-truth intent labels, such as \textit{PlayMusic}, \textit{RateBook}, etc. 
The SNIPS dataset is a good candidate to evaluate the proposed approach, since the manual intent labels generally follow an ACTION-OBJECT pattern and all the intents have similar numbers of utterances (cv=0.26). Note that these intent labels are only used for performance evaluation in our experiments.

For unsupervised clustering, we obtain the semantic representation of each sentence from 4 different models, as shown in Table~\ref{tab:representations}. The first three models are pre-trained using the SBERT model \cite{reimers2019sentencebert} with various pre-trained tasks using different datasets, while the fourth is called Universal Sentence Encoder \cite{cer2018universal}, which is pre-trained from a variety of web sources such as Wikipedia, web news, discussion forums and achieves superior performance on the semantic textual similarity task.
\vspace{-0.5em}
\begin{table}[htb]
\centering
\caption{Pre-trained sentence representation models.}
\vspace{-0.5em}
\label{tab:representations}
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|ll}
\hline
\textbf{Name} & \textbf{Pre-trained Model} & \textbf{Training Objective} \\ \hline
% glove & avg-glove.6B.300d & GloVe & Wikipedia+Gigaword \\
nli-bert & nli-bert-base-max-pooling & natural language inference \\
% stsb-bert & stsb-bert-base & bert-base-uncased & NLI+STSb \\
stsb-bert & stsb-roberta-base & semantic textual similarity \\
paraphrase & paraphrase-distilroberta-base-v1 & paraphrase identification \\
universal & universal sentence encoder & unsupervised \& NLI \\ \hline
\end{tabular}%
}
\end{table}

\vspace{-1em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation Metrics}
Since the SNIPS dataset has ground-truth intent labels, we adopt precision (P), recall (R) and $F_1$ to evaluate the proposed intent discovery framework.
Following \cite{chatterjee2020intent}, we also use the Normalized Mutual Information (NMI \cite{knops2006normalized}) and Adjusted Rand Index (ARI \cite{rand1971objective}) as the metrics for evaluating clustering performance.
NMI normalizes the mutual information between a predicted clustering and the true clustering, and ranges from 0 to 1; while ARI computes the similarity between two clusterings by considering all pairs of examples and counting the proportion of pairs that are assigned to the same or different clusters.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results and Analysis}
% In this Section, we first illustrate the unsupervised clustering stage, and then show the label generation process, and finally present the evaluation results quantitatively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Stage I: Unsupervised Clustering}

\noindent\textbf{Effect of \textit{Balanced Score}.}
We adopt $K$-means for clustering and determine the number of clusters based on the metric of \textit{balanced score}.
As compared in Figure~\ref{fig:k-clusters}, using the balanced score leads to the correct number of clusters, (i.e., \textbf{7}) for either the \texttt{paraphrase} or \texttt{universal} representation, while the Silhouette score gives a correct $K$ only for the \texttt{paraphrase} representation.
Besides, the Silhouette score tends to have a level curve with slight changes under different $K$, while the balanced score changes dramatically since it gives higher penalty if a $K$ value leads to more unbalanced clusters.
We set $\lambda$ as 0.5 for computing the balanced scores in our experiments.

\vspace{-1em}
\begin{figure}[htb]
\centering
\begin{subfigure}{0.22\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/scores/nli-bert.pdf}
  \caption{nli-bert}
  \label{fig:nli}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/scores/stsb-bert.pdf}
  \caption{stsb-bert}
  \label{fig:stsb}
\end{subfigure}%

\begin{subfigure}{0.22\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/scores/paraphrase.pdf}
  \caption{paraphrase}
  \label{fig:paraphrase}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/scores/use.pdf}
  \caption{universal}
  \label{fig:use}
\end{subfigure}%
\caption{Changes of the Silhouette score and balanced score with different number of clusters using different representations.}
\label{fig:k-clusters}
\end{figure}


\noindent\textbf{Cluster Visualization.}
For qualitative comparison, we visualize the four types of semantic representations using t-SNE\cite{van2008visualizing}, where different colors represent different clusters. 
It can be seen that the \texttt{paraphrase} representation has better cluster separations than both \textit{nli-bert} and \textit{stsb-bert}, while the clusters using the \texttt{universal} representation show the best separations.
\begin{figure*}[htb]
\centering
\begin{subfigure}{0.23\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/tsne/nli-bert.pdf}
  \caption{nli-bert}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{0.23\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/tsne/stsb-bert.pdf}
  \caption{stsb-bert}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{0.23\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/tsne/paraphrase.pdf}
  \caption{paraphrase}
  \label{fig:sfig4}
\end{subfigure}
\begin{subfigure}{0.23\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/tsne/use.pdf}
  \caption{universal}
  \label{fig:tsne-use}
\end{subfigure}%
\caption{t-SNE visualization of clusters using different representations. The utterance percentage of each cluster is also shown.}
\label{fig:clusters}
\end{figure*}


\begin{table*}[htb]
\centering
\caption{Results of intent label generation by a dependency parser from the clusters obtained using the \textit{universal} representation.}
\label{tab:label-generation}
\resizebox{0.96\textwidth}{!}{%
\begin{tabular}{clrlrr}
\hline
\textbf{Cluster} & \multicolumn{1}{c}{\textbf{Top 3 ACTION-OBJECT pairs}} & \multicolumn{1}{c}{\textbf{Percentage}} & \multicolumn{1}{c}{\textbf{Example Utterance}} & \multicolumn{1}{r}{\textbf{Generated}} & \multicolumn{1}{r}{\textbf{Ground-truth}} \\ \hline
0 & ('book-restaurant', 313), ('book-table', 281), ('book-spot', 131) & 36.90\% & i want to \textbf{book} a \textbf{restaurant} for nine with wifi & book-restaurant & BookRestaurant \\
1 & ('find-schedule', 164), ('be-schedule', 100), ('show-schedule', 98) & 22.14\% & \textbf{find} the movie \textbf{schedule} for close by films & find-schedule & SearchScreeningEvent \\
2 & ('add-tune', 160), ('add-song', 150), ('add-track', 134) & 22.57\% & \textbf{add} \textbf{tune} to sxsw fresh playlist & add-tune & AddToPlaylist \\
3 & ('find-show', 82), ('find-game', 50), ('show-creativity', 42) & 7.46\% & can you \textbf{find} me the spectres television \textbf{show} ? & find-show & SearchCreativeWork \\
4 & ('give-star', 133), ('rate-book', 104), ('rate-novel', 82) & 16.87\% & i \textbf{give} 4 of 6 \textbf{stars} for the saga severe mercy & give-star & RateBook \\
5 & ('be-weather', 395), ('be-forecast', 330), ('tell-forecast', 54) & 37.60\% & what \textbf{is} the \textbf{weather} for my current place & be-weather & GetWeather \\
6 & ('play-music', 424), ('play-song', 198), ('play-track', 75) & 36.28\% & please \textbf{play} some bill evans \textbf{music} & play-music & PlayMusic \\ \hline
\end{tabular}%
}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Stage II: Intent Label Generation}

Based on the clustering results from Stage I, we adopt a dependency parser to extract the ACTION-OBJECT pair for each utterance within each cluster.
Table~\ref{tab:label-generation} shows the top 3 ACTION-OBJECT pairs and the number of utterances having these pairs within each cluster, where the clustering results are obtained using the best \texttt{universal} representation. The third column presents the percentage of utterances covering the top 3 ACTION-OBJECT pairs. A higher percentage means the pair is more representative of the cluster.
Referring to each example utterance, it is observable to see that these pairs are meaningful labels for the clusters and match well with the ground-truth labels.
Note that although some datasets may not exhibit such ACTION-OBJECT patterns for intent labels, e.g., the very short informal conversations, the first stage of the framework is still applicable for identifying the unknown intents from the dataset and estimate the number of possible intents which can be very large in some complex datasets.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Quantitative Evaluation}
Since the SNIPS dataset has ground-truth labels, we evaluate the proposed two-stage framework quantitatively by comparing the performance among the semantic representations and presenting the intent-level performance based on the best \texttt{universal} representation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Representation Comparisons.}
Recall that the representations are pre-trained on various datasets using different training objectives, hence, they may give different performance in the semantic clustering stage.
Table~\ref{tab:performance} shows the performance comparisons among different representations on the SNIPS dataset. It is clear that the pre-trained \texttt{universal} representation obtains the best performance on all the metrics.
This is also consistent with the cluster visualization results shown in Figure~\ref{fig:clusters}.

% \vspace{-0.5em}
\begin{table}[htb]
\centering
\caption{Performance comparisons among representations.}
\label{tab:performance}
\resizebox{0.86\linewidth}{!}{%
\begin{tabular}{r|ccccc}
\hline
\textbf{Representation} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{NMI}} & \multicolumn{1}{c}{\textbf{ARI}} \\ \hline
nli-bert & 0.682 & 0.635 & 0.647 & 0.597 & 0.505 \\
stsb-bert & 0.725 & 0.682 & 0.688 & 0.665 & 0.565 \\
paraphrase & 0.923 & 0.928 & 0.924 & 0.835 & 0.831 \\
universal & \textbf{0.934} & \textbf{0.940} & \textbf{0.935} & \textbf{0.865} & \textbf{0.855} \\ \hline
\end{tabular}%
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Intent-level Performance.}
% Since the SNIPS dataset has ground-truth labels, we can evaluate the proposed two-stage approach quantitatively.
We report the intent-level performance on the SNIPS dataset based on the \texttt{universal} representation.
As shown in Table~\ref{tab:snips}, all the intents have been successfully discovered and each ground-truth intent is semantically mapped to the corresponding generated intent label. Moreover, good performance is achieved for all the intents, since the universal representation can separate the utterances clearly.
We attribute the good clustering performance to the pre-trained models for obtaining semantic representations, and the metric of \textit{balanced score} in determining the number of clusters.

% \vspace{-0.5em}
\begin{table}[htb]
\centering
\caption{Intent-level performance on the SNIPS dataset using the \texttt{universal} representation.}
\label{tab:snips}
\resizebox{0.86\linewidth}{!}{%
\begin{tabular}{r|r|ccc}
\hline
\textbf{Ground-truth} & \textbf{Generated} & \textbf{P} & \textbf{R} & \textbf{$F_1$} \\ \hline
AddToPlaylist & add-tune & 0.954 & 0.942 & 0.948 \\
BookRestaurant & book-restaurant & 0.987 & 0.991 & 0.989 \\
GetWeather & be-weather & 0.989 & 0.954 & 0.971 \\
PlayMusic & play-music & 0.894 & 0.931 & 0.912 \\
RateBook & give-star & 0.965 & 0.998 & 0.982 \\
SearchCreativeWork & find-show & 0.924 & 0.774 & 0.843 \\
SearchScreeningEvent & find-schedule & 0.826 & 0.990 & 0.901 \\ \hline
\multicolumn{2}{r|}{Average} & 0.934 & 0.940 & 0.935 \\ \hline
\end{tabular}%
}
\end{table}


==> intent-discovery-archive/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}

The critical first step towards goal-oriented dialog systems is to determine the goal and the corresponding ontologies consisting of intents and slots that define the natural language understanding (NLU) targets. The process of intent recognition and slot filling are typically formulated as supervised classification problems which has been extensively studied to achieve high performance in closed-domain datasets, where the training samples are usually hand-labelled. However, in a real-world dialog system, such as a customer support application \cite{perkins2019dialog}, the domain is usually open and more complex which pose difficulties in manually labelling accurate intents and slots, not to mention that the volume of conversational data may be very large. Therefore, it is desirable to find an automatic method to identify the intents and slots from raw conversational data, in order to reduce the cost of manual data annotation.

This paper focuses on the problem of \textit{unsupervised open intent discovery} which involves two sub-tasks: (1) automatically discover all intents from a corpus of goal-oriented dialog, and (2) automatically assign each utterance in the dialog corpus to the discovered intent. Such a problem is very challenging as the intents discovered need to be consistent with human understanding, hence each discovered intent should be labelled with an interpretable name. We also observe that it is common in conversational datasets for an utterance to be composed of an ACTION-OBJECT pattern. For example, in the utterance ``\textit{Could you please help me book a flight from Beijing to Shanghai?}", the pair can be defined as (book, flight) which can form a label reflecting the intent, i.e. \textit{book-flight}.

We propose an unsupervised data-driven framework for open intent discovery, leveraging recent advances in pre-trained language models \cite{pennington2014glove,peters2018deep,devlin2018bert}. First, we obtain the semantic representation of each utterance using the pre-trained model so that all utterances in the corpus can be represented by points lying in the semantic space. Second, we apply a clustering technique to group the utterances based on their semantic representations by assuming that the utterances of the same intent are close to each other in the semantic space. To better estimate the number of clusters, we introduce a novel metric named \textit{balanced score} which is found to be particularly useful for datasets with intents having similar number of samples. Third, we generate the intent label that are interpretable using the most frequent ACTION-OBJECT pair within each cluster. The ACTION-OBJECT pair for each utterance can be extracted by a dependency parser. We found that the experimental results on the SNIPS dataset are surprisingly good, where the discovered intents match with all the ground-truth intent labels, and the sub-task of assigning each utterance to the appropriate intent achieves a high $F_1$ score of 93\%. 
% We also show that the proposed framework is flexible by adopting different pre-trained language models.
The contributions of this paper are three-fold:
\begin{enumerate}[(1)]
\item We propose a flexible framework for open intent discovery which can generate human-interpretable intents, and label the utterances with a high $F_1$ in an unsupervised manner; % while achieving a high $F_1$;
\item We develop a rule-based approach for generating intent labels automatically using dependency parsing;
\item We enhance the standard $K$-means clustering in determining the optimal number of clusters for a balanced dataset using a newly proposed \textit{balanced score} metric.
\end{enumerate}


==> intent-discovery-archive/related.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}

The problem of \textit{open intent discovery} is closely related with intent recognition, semantic representation and unsupervised clustering. Intent recognition aims to identify the intent expressed in an utterance, e.g., the intent of \textit{buy-computer} in the utterance of ``\texttt{I want to buy a new computer}". This is an important task widely applicable in goal-oriented dialog systems, conversation analysis and online advertisement, and supervised learning methods \cite{tur2011intent,liu2016attention,meng2017dialogue,schuurmans2019intent,khalil2019cross,wang2020dialogue,firdaus2020deep,zhang2016joint} are typically adopted to learn classifiers from labeled intent datasets.
According to the different application scenarios, intent recognition can be categorized into (1) query intent classification (e.g., a search engine \cite{jansen2007determining,cao2009context,strohmaier2012acquiring}); (2) intent identification from social media (e.g. Twitter messages) \cite{ashkan2009term,wang2013mining}; (3) user intent understanding in a dialog system \cite{liu2016attention,goo2018slot,niu2019novel}.


Semantic representation in the context of natural language processing typically refers to continuous vectors capturing the meaning of words, phrases or utterances. They are typically learned from a large collection of text corpora, e.g., word2vec\cite{mikolov2013distributed}, Glove\cite{pennington2014glove}, Elmo\cite{peters2018deep}, BERT\cite{devlin2018bert}, etc.
Unsupervised clustering groups a collection of unlabeled examples into a set of clusters, where the examples within each cluster share similar semantics. Typical clustering methods include $K$-means\cite{macqueen1967some}, Gaussian mixture models\cite{reynolds2009gaussian}, DBSCAN\cite{ester1996density}, etc. 
% One of the challenges is to determine the number of clusters, although there are a few techniques such as Silhoueete score\cite{rousseeuw1987silhouettes}.
One of the key challenges is to determine the number of clusters, although some have used graphical aids such as the Silhouette score\cite{rousseeuw1987silhouettes}.


Typical approaches to open intent discovery include supervised learning methods, semi-supervised learning methods and unsupervised learning methods.
For example, Vedula et al. \cite{vedula2019towards} proposes a two-stage approach for the task of open intent discovery by first predicting the existence of an intent in an utterance and then tagging utterance with the labels of \textit{Action, Object, and None} using a BiLSTM-CRF model. However, this approach needs a labeled dataset.
Alternatively, Cai et al.\cite{cai2017cnn} adopts a hierarchical clustering method to learn user intent taxonomy, where an intent is represented by a concept pair \textit{(disease, reason)} for a user utterance from online health communities, and proposes a CNN-LSTM attention model to predict user intent.
To address the challenge of the lack of labeled intent datasets, Wang et al.\cite{wang2015mining} introduces a graph-based semi-supervised learning approach to categorize intent tweets into six predefined categories. Unlike the setting in unsupervised learning setting, this approach needs a small number of labeled tweets and a set of intent keywords as input.


From the perspective of unsupervised learning, Perkins and Yang \cite{perkins2019dialog} presents an algorithm named \textit{alternating-view k-means} to discover user intents from query utterances in human-human conversations.
To leverage the whole dialog content, this algorithm divides a dialog into a query view and a content view, which are encoded by two separate neural encoders. The two encoders are updated iteratively using the cluster assignment obtained from the alternative view to encourage them to yield similar cluster assignments for the same user queries.
% Haponchyk et al. \cite{haponchyk2018supervised}
Along the direction of unsupervised clustering approaches, Chatterjee and Sengupta \cite{chatterjee2020intent} present an intent discovery framework for conversation data, which consists of dialog act classification, density-based clustering, manual annotation of clusters and propagation of intent labels. In comparison with previous approaches, this work differs in three major aspects: (1) we adopt pre-trained language models for utterance representation; (2) we incorporate $K$-means with a penalty term to learn the optimal number of clusters; and (3) we generate the cluster labels automatically using a dependency parser. 


